On the choice of initial guesses for the Newton-Raphson algorithm

The initialization of equation-based differential-algebraic system models, and more in general the solution of many engineering and scientific problems, require the solution of systems of nonlinear equations. Newton-Raphson's method is widely used for this purpose; it is very efficient in the computation of the solution if the initial guess is close enough to it, but it can fail otherwise. In this paper, several criteria are introduced to analyze the influence of the initial guess on the evolution of Newton-Raphson's algorithm and to identify which initial guesses need to be improved in case of convergence failure. In particular, indicators based on first and second derivatives of the residual function are introduced, whose values allow to assess how much the initial guess of each variable can be responsible for the convergence failure. The use of such criteria, which are based on rigorously proven results, is successfully demonstrated in three exemplary test cases.

==> DC_log.tex <==
Initial values and first increment:
w_0  =      0.99999       0.69999      10.69989  
dw_0 =      0.00001       0.00001       0.00011  

Non-zero Gamma values:
$ \Gamma_{122} = 0.000 $
$ \Gamma_{213} = 0.000 $

Non-zero alpha values:
$ \alpha_{1} = 1.36e-08

Sigma = 
      -0.000 &        0.000 &       -0.000 \\
      -0.000 &       -0.000 &       -0.000 \\
      -0.000 &       -0.000 &       -0.000 \\

SUCCESS: Newton-Raphson algorithm converged in 2 iterations!

Initial values and first increment:
w_0  =      0.99000       0.69300      10.59300  
dw_0 =      0.01000       0.00808       0.10808  

Non-zero Gamma values:
$ \Gamma_{122} = 0.168 $
$ \Gamma_{213} = 0.002 $

Non-zero alpha values:
$ \alpha_{1} =   0.0197

Sigma = 
      -0.005 &        0.013 &       -0.005 \\
      -0.000 &       -0.323 &       -0.000 \\
      -0.005 &       -0.012 &       -0.005 \\

SUCCESS: Newton-Raphson algorithm converged in 4 iterations!

Initial values and first increment:
w_0  =      0.90000       0.63000       9.63000  
dw_0 =      0.09066       0.38228       1.28885  

Non-zero Gamma values:
$ \Gamma_{122} = 3.497 $
$ \Gamma_{213} = 0.029 $

Non-zero alpha values:
$ \alpha_{1} = 1.31e+05

Sigma = 
      -0.068 &        3.054 &       -0.068 \\
      -0.007 &      -14.993 &       -0.007 \\
      -0.050 &       -2.299 &       -0.050 \\

SUCCESS: Newton-Raphson algorithm converged in 18 iterations!

Initial values and first increment:
w_0  =      0.80000       0.56000       8.56000  
dw_0 =     -0.02070       5.24356       5.03653  

Non-zero Gamma values:
$ \Gamma_{122} =21.116 $
$ \Gamma_{213} = 0.014 $

Non-zero alpha values:
$ \alpha_{1} = 1.18e+88

Sigma = 
       0.229 &     1934.463 &        0.229 \\
       0.006 &     -158.105 &        0.006 \\
       0.016 &      -85.085 &        0.016 \\

WARNING: Newton-Raphson algorithm did not converge!

Initial values and first increment:
w_0  =      0.25000       0.69300       2.67500  
dw_0 =      1.91114       0.04649      19.67585  

Non-zero Gamma values:
$ \Gamma_{122} = 0.067 $
$ \Gamma_{213} = 0.958 $

Non-zero alpha values:
$ \alpha_{1} =   0.0705

Sigma = 
      -3.796 &        0.002 &       -3.796 \\
      -5.162 &       -1.856 &       -5.162 \\
      -3.699 &       -0.002 &       -3.699 \\

SUCCESS: Newton-Raphson algorithm converged in 7 iterations!

$\alpha_{1}$   & 0.000 & 0.020 & 1.31e+05 & 1.18e+88 & 0.071 \\
$\Gamma_{122}$ & 0.000 & 0.168 &    3.497 &   21.116 & 0.067 \\
$\Gamma_{213}$ & 0.000 & 0.002 &    0.029 &    0.014 & 0.958 \\


==> FTD_log.tex <==
Initial values and first increment:
w_0  =      0.99999       0.99999       3.99996       0.99999       1.99998       2.19998  
dw_0 =      0.00001       0.00001       0.00004       0.00001       0.00002       0.00002  

Non-zero Gamma values:
$ \Gamma_{166} = 0.005 $
$ \Gamma_{211} = 0.000 $
$ \Gamma_{325} = 0.000 $
$ \Gamma_{355} = 0.000 $
$ \Gamma_{413} = 0.000 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.000 $

Non-zero alpha values:
$ \alpha_{1} = 4.91e-05

Sigma = 
      -0.000 &        0.000 &        0.000 &        0.000 &        0.000 &        0.000 \\
      -0.000 &       -0.000 &        0.000 &        0.000 &        0.000 &        0.010 \\
      -0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.000 \\
      -0.000 &        0.000 &        0.000 &        0.000 &        0.000 &       -0.000 \\
      -0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.010 \\
       0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.010 \\

SUCCESS: Newton-Raphson algorithm converged in 3 iterations!

Initial values and first increment:
w_0  =      0.99900       0.99900       3.99600       0.99900       1.99800       2.19800  
dw_0 =      0.00100       0.00073       0.00400       0.00100       0.00254       0.00254  

Non-zero Gamma values:
$ \Gamma_{166} = 0.211 $
$ \Gamma_{211} = 0.000 $
$ \Gamma_{325} = 0.000 $
$ \Gamma_{355} = 0.000 $
$ \Gamma_{413} = 0.000 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.000 $

Non-zero alpha values:
$ \alpha_{1} =    0.224

Sigma = 
      -0.000 &        0.000 &        0.000 &        0.000 &        0.000 &       -0.000 \\
      -0.000 &       -0.001 &        0.000 &        0.001 &        0.001 &        0.733 \\
      -0.001 &        0.000 &       -0.001 &       -0.000 &        0.000 &        0.000 \\
      -0.000 &        0.000 &        0.000 &        0.000 &        0.000 &        0.000 \\
      -0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.423 \\
       0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.423 \\

SUCCESS: Newton-Raphson algorithm converged in 5 iterations!

Initial values and first increment:
w_0  =      0.99000       0.99000       3.96000       0.99000       1.98000       2.17800  
dw_0 =      0.00999       0.00276       0.04043       0.01000       0.03443       0.03641  

Non-zero Gamma values:
$ \Gamma_{166} = 0.395 $
$ \Gamma_{211} = 0.000 $
$ \Gamma_{325} = 0.000 $
$ \Gamma_{355} = 0.000 $
$ \Gamma_{413} = 0.000 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.000 $

Error: negative square root
Error: negative square root

Reduction of newton step necessary:
lambda=0.490

Non-zero alpha values:
$ \alpha_{1} =    0.678
$ \alpha_{3} = 5.81e-07

Sigma = 
      -0.003 &        0.000 &        0.000 &        0.004 &        0.000 &        0.000 \\
      -0.004 &       -0.018 &        0.000 &        0.017 &        0.093 &        5.283 \\
      -0.007 &        0.000 &       -0.010 &       -0.004 &        0.000 &       -0.000 \\
      -0.004 &        0.000 &        0.000 &        0.003 &        0.000 &       -0.000 \\
      -0.001 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.837 \\
       0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.791 \\

Error: negative square root
NR algorithm stopped

Initial values and first increment:
w_0  =      0.90000       0.90000       3.60000       0.90000       1.80000       1.98000  
dw_0 =      0.09930      -0.00468       0.44724       0.10030       0.39454       0.41229  

Non-zero Gamma values:
$ \Gamma_{166} = 0.463 $
$ \Gamma_{211} = 0.001 $
$ \Gamma_{325} = 0.000 $
$ \Gamma_{355} = 0.002 $
$ \Gamma_{413} = 0.000 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.000 $

Error: negative square root
Error: negative square root

Reduction of newton step necessary:
lambda=0.490

Non-zero alpha values:
$ \alpha_{1} =     1.32
$ \alpha_{3} = 0.000384
$ \alpha_{6} = 2.75e-06

Sigma = 
      -0.028 &        0.000 &        0.000 &        0.043 &        0.000 &       -0.000 \\
      -0.328 &        0.247 &        0.012 &        1.226 &       11.951 &       46.268 \\
      -0.085 &        0.000 &       -0.111 &       -0.038 &        0.000 &        0.000 \\
      -0.041 &        0.000 &        0.000 &        0.035 &        0.000 &        0.000 \\
      -0.007 &        0.000 &       -0.000 &       -0.004 &        0.000 &       -0.975 \\
       0.000 &        0.000 &       -0.000 &       -0.000 &        0.000 &       -0.933 \\

Error: negative square root
NR algorithm stopped

Initial values and first increment:
w_0  =      0.90000       0.90000       3.60000       0.90000       1.80000       2.15100  
dw_0 =      0.09930       0.08275       0.44724       0.10030       0.23912       0.08587  

Non-zero Gamma values:
$ \Gamma_{166} = 0.422 $
$ \Gamma_{211} = 0.002 $
$ \Gamma_{325} = 0.001 $
$ \Gamma_{355} = 0.001 $
$ \Gamma_{413} = 0.001 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.000 $

Error: negative square root
Error: negative square root

Reduction of newton step necessary:
lambda=0.490

Non-zero alpha values:
$ \alpha_{1} =    0.902
$ \alpha_{3} = 7.47e-05
$ \alpha_{6} = 6.22e-06

Sigma = 
      -0.028 &        0.000 &        0.000 &        0.043 &        0.000 &       -0.000 \\
      -0.018 &       -0.149 &        0.001 &        0.069 &        0.093 &        0.501 \\
      -0.085 &        0.000 &       -0.111 &       -0.038 &        0.000 &        0.000 \\
      -0.041 &        0.000 &        0.000 &        0.035 &        0.000 &        0.000 \\
      -0.012 &        0.000 &       -0.000 &       -0.007 &        0.000 &       -0.308 \\
       0.000 &        0.000 &       -0.000 &       -0.001 &        0.000 &       -0.859 \\

Error: negative square root
NR algorithm stopped

Initial values and first increment:
w_0  =      3.00000       0.99900       3.99600       0.99900       1.99800       2.19800  
dw_0 =     -2.15359      -0.64593       0.20592       0.02620       0.98738       0.00307  

Non-zero Gamma values:
$ \Gamma_{166} = 0.028 $
$ \Gamma_{211} = 0.580 $
$ \Gamma_{325} = 0.020 $
$ \Gamma_{355} = 0.015 $
$ \Gamma_{413} = 0.007 $
$ \Gamma_{534} = 0.000 $
$ \Gamma_{611} = 0.012 $

Error: negative square root

Reduction of newton step necessary:
lambda=0.700

Non-zero alpha values:
$ \alpha_{1} =   0.0284
$ \alpha_{3} =   0.0128
$ \alpha_{6} =  0.00505

Sigma = 
       0.125 &        0.000 &        0.011 &        0.000 &        0.000 &       -0.000 \\
       2.104 &        0.495 &        0.059 &        0.002 &        0.873 &        0.001 \\
      -1.019 &        0.000 &        0.565 &       -0.005 &        0.000 &        0.000 \\
      -0.999 &        0.000 &        0.580 &        0.020 &        0.000 &        0.000 \\
      -2.206 &        0.000 &       -0.029 &       -0.001 &        0.000 &       -0.002 \\
      -0.303 &        0.000 &       -0.027 &       -0.001 &        0.000 &       -0.511 \\

Error: negative square root
NR algorithm stopped

$\alpha_{1}$   & 0.000 & 0.224 & 0.678 & 1.316 & 0.902 & 0.028 \\
$\alpha_{3}$   & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.013 \\
$\alpha_{6}$   & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 \\
$\Gamma_{166}$ & 0.005 & 0.211 & 0.395 & 0.463 & 0.422 & 0.028 \\
$\Gamma_{211}$ & 0.000 & 0.000 & 0.000 & 0.001 & 0.002 & 0.580 \\
$\Gamma_{325}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.020 \\
$\Gamma_{355}$ & 0.000 & 0.000 & 0.000 & 0.002 & 0.001 & 0.015 \\
$\Gamma_{413}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.007 \\
$\Gamma_{534}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
$\Gamma_{611}$ & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 \\

